Flattenicity as "centrality" estimator in p-Pb collisions simulated with PYTHIA 8.312 Angantyr

In this paper, a "centrality" estimator based on flattenicity ($\rho$) is studied in proton-led (p-Pb) collisions at $\sqrt{s_{\rm NN}}=5.02$ TeV using PYTHIA 8 Angantyr. Although Angantyr is still under development, the existing implementation is enough to study the particle production in systems where medium effects are absent. Firstly, ALICE data on pseudorapidity distributions as a function of the forward multiplicity (V0M), as well as transverse momentum distributions of identified particles in non-single diffractive p-Pb collisions, are compared with Angantyr. Secondly, the average number of binary nucleon-nucleon ($N_{\rm coll}$) collisions for different "centrality" estimators are compared. The studies include the following "centrality" estimators: V0M, $\rho$ and midrapidity multiplicity (CL1). On one hand, the "centrality" dependence of $\langle N_{\rm coll} \rangle$ for the $\rho$ selection shows the smallest deviations ($<8$ %) with respect to that obtained using impact parameter $b$; on the other hand, the V0M and CL1 yield huge deviations (up to a factor 2) with respect to the results using $b$. The particle ratios and nuclear modification factors ($Q_{\rm pPb}$) as a function of $p_{\rm T}$ are also studied. The proton-to-pion ratio exhibits a flow-like peak at intermediate $p_{\rm T}$ (2-8 GeV/$c$) with little or no "centrality" dependence for V0M, $\rho$ and $b$ selections. The kaon-to-pion ratio as a function of $p_{\rm T}$ is "centrality" independent for the same selections. On the contrary, for the CL1 class the ratios exhibit the typical behaviour associated with hard physics. Regarding $Q_{\rm pPb}$, a peak at intermediate $p_{\rm T}$ ($2-8$ GeV/$c$) for different particle species is observed when the "centrality" is obtained with $b$ or $\rho$. The observed features diminish for the selections based on V0M and CL1.

==> commands.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% These are some new commands that may be useful 
% for paper writing in general. If other newcommands
% are needed for your specific paper, please feel 
% free to add here. 
%
% The currently available commands are organized in: 
% 1) Systems
% 2) Quantities
% 3) Energies and units
% 4) Detectors
% 5) particle species 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\red}{\textcolor{red}}
\newcommand{\blue}{\textcolor{blue}}

%%%%%%%%%%%%%%%  Command definition %%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\orho}{\ensuremath{1-\rho}\xspace}
\newcommand{\Rpp}{\ensuremath{R_{\mathrm{pp}}}\xspace}

\newcommand{\ST}{\ensuremath{S_{\rm T}}\xspace}
\newcommand{\RT}{\ensuremath{R_{\rm T}}\xspace}
\newcommand{\Nm}{\ensuremath{N_{\mathrm{m}}}\xspace}
\newcommand{\Nt}{\ensuremath{N_{\mathrm{t}}}\xspace}
%\newcommand{\NT}{\ensuremath{N_{\mathrm{T}}}\xspace}
\newcommand{\mNT}{\ensuremath{\langle N_{\mathrm{T}}} \rangle \xspace}
\newcommand{\Smt}{\ensuremath{S_{\mathrm{mt}}}\xspace}

\newcommand{\pipm}{\ensuremath{\pi^{\pm}}\xspace}
\newcommand{\kpm}{\ensuremath{\mathrm{K}^{\pm}}\xspace}
\newcommand{\ppm}{\ensuremath{(\overline{\mathrm{p}})\mathrm{p}}\xspace}


% Unfolding

\newcommand{\RMp}{\ensuremath{P(N_{\mathrm{T,m}}|N_{\mathrm{T,t}})}\xspace}
\newcommand{\NTc}{\ensuremath{N_{\mathrm{T}}}\xspace}
\newcommand{\NTt}{\ensuremath{N_{\mathrm{T,t}}}\xspace}
\newcommand{\NTm}{\ensuremath{N_{\mathrm{T,m}}}\xspace}
\newcommand{\UM}{\ensuremath{M_{\mathrm{tm}}}\xspace}

\newcommand{\UnfDis}{\ensuremath{Y(N_{\mathrm{T,t}}})\xspace}
\newcommand{\RawDis}{\ensuremath{Y(N_{\mathrm{T,m}}})\xspace}
\newcommand{\Mone}{\ensuremath{\mathrm{M1}_{\mathrm{tm}}}\xspace}
\newcommand{\Mtwo}{\ensuremath{\mathrm{M2}_{\mathrm{tm}}(p_{\mathrm{T}})}\xspace}
\newcommand{\Prior}{\ensuremath{P_{0}(\NTm)}\xspace}
\newcommand{\UpdatedPrior}{\ensuremath{\widehat{P}(\NTt)}\xspace}
\newcommand{\RawYield}{\ensuremath{\mathrm{d}Y(N_{\mathrm{T,m}})/\mathrm{d}p_{\mathrm{T}}}}
\newcommand{\UnfYield}{\ensuremath{\mathrm{d}Y(N_{\mathrm{T,t}})/\mathrm{d}p_{\mathrm{T}}}}

\newcommand{\dndetainline}{\ensuremath{\langle\text{d}N_{\rm{ch}}/\text{d}\eta\rangle}\xspace}
\newcommand{\dndyinline}{\ensuremath{\text{d}N/\text{d}y}\xspace}
\newcommand{\dndydptinline}{\ensuremath{\text{d}^2N/\text{d}\ptt \text{d}y}\xspace}

% 1) SYSTEMS 
\newcommand{\pp}           {pp\xspace}
\newcommand{\ppbar}        {\mbox{$\mathrm {p\overline{p}}$}\xspace}
\newcommand{\XeXe}         {\mbox{Xe--Xe}\xspace}
\newcommand{\PbPb}         {\mbox{Pb--Pb}\xspace}
\newcommand{\pA}           {\mbox{pA}\xspace}
\newcommand{\pPb}          {\mbox{p--Pb}\xspace}
\newcommand{\AuAu}         {\mbox{Au--Au}\xspace}
\newcommand{\dAu}          {\mbox{d--Au}\xspace}

% 2) QUANTITIES 
\newcommand{\s}            {\ensuremath{\sqrt{s}}\xspace}
\newcommand{\snn}          {\ensuremath{\sqrt{s_{\mathrm{NN}}}}\xspace}
%\newcommand{\pt}           {\ensuremath{p_{\rm T}}\xspace}
\newcommand{\mt}           {\ensuremath{m_{\mathrm{T}}}\xspace}
\newcommand{\ptleading}    {\ensuremath{p_{\rm T}^{\rm{leading}}}\xspace}
\newcommand{\meanpt}       {\ensuremath{\langle p_{\rm T}\rangle}\xspace}
\newcommand{\ycms}         {\ensuremath{y_{\rm CMS}}\xspace}
\newcommand{\ylab}         {\ensuremath{y_{\rm lab}}\xspace}
\newcommand{\etarange}[1]  {\mbox{$\left | \eta \right |~<~#1$}}
\newcommand{\yrange}[1]    {\mbox{$\left | y \right |~<~#1$}}
\newcommand{\dndy}         {\ensuremath{\mathrm{d}N/\mathrm{d}y}\xspace}
\newcommand{\dndeta}       {\ensuremath{\mathrm{d}N_\mathrm{ch}/\mathrm{d}\eta}\xspace}
\newcommand{\avdndeta}     {\ensuremath{\langle\dndeta\rangle}\xspace}
\newcommand{\dNdy}         {\ensuremath{\mathrm{d}N_\mathrm{ch}/\mathrm{d}y}\xspace}
\newcommand{\Npart}        {\ensuremath{N_\mathrm{part}}\xspace}
\newcommand{\Ncoll}        {\ensuremath{N_\mathrm{coll}}\xspace}
\newcommand{\dEdx}         {\ensuremath{\textrm{d}E/\textrm{d}x}\xspace}
\newcommand{\meandEdx}{\ensuremath{\langle\textrm{d}E/\textrm{d}x}\rangle\xspace}

\newcommand{\RpPb}         {\ensuremath{R_{\rm pPb}}\xspace}
\newcommand{\Qpp}         {\ensuremath{Q_{\rm pp}}\xspace}


% 3) ENERGIES, UNITS
\newcommand{\nineH}        {$\sqrt{s}~=~0.9$~Te\kern-.1emV\xspace}
\newcommand{\seven}        {$\sqrt{s}~=~7$~Te\kern-.1emV\xspace}
\newcommand{\twoH}         {$\sqrt{s}~=~0.2$~Te\kern-.1emV\xspace}
\newcommand{\twosevensix}  {$\sqrt{s}~=~2.76$~Te\kern-.1emV\xspace}
\newcommand{\five}         {$\sqrt{s}~=~5.02$~Te\kern-.1emV\xspace}
\newcommand{\thirteen}    {$\sqrt{s}~=~13$~Te\kern-.1emV\xspace}
\newcommand{\twosevensixnn}{$\sqrt{s_{\mathrm{NN}}}~=~2.76$~Te\kern-.1emV\xspace}
\newcommand{\fivenn}       {$\sqrt{s_{\mathrm{NN}}}~=~5.02$~Te\kern-.1emV\xspace}
\newcommand{\LT}           {L{\'e}vy-Tsallis\xspace}
\newcommand{\GeVc}         {Ge\kern-.1emV/$c$\xspace}
\newcommand{\MeVc}         {Me\kern-.1emV/$c$\xspace}
\newcommand{\TeV}          {Te\kern-.1emV\xspace}
\newcommand{\GeV}          {Ge\kern-.1emV\xspace}
\newcommand{\MeV}          {Me\kern-.1emV\xspace}
\newcommand{\GeVmass}      {Ge\kern-.2emV/$c^2$\xspace}
\newcommand{\MeVmass}      {Me\kern-.2emV/$c^2$\xspace}
\newcommand{\lumi}         {\ensuremath{\mathcal{L}}\xspace}
%\newcommand{\gevc}         {\ensuremath{\mathrm{GeV}/c}\xspace}
\newcommand{\gevc}[1]      {\ensuremath{#1 \text{\,GeV/$c$}}\xspace}
\newcommand{\mevc}[1]      {\ensuremath{#1 \text{\,MeV/$c$}}\xspace}
\newcommand{\sppt}[1]      {\ensuremath{\sqrt{s} = #1 \text{\,TeV}}\xspace}


% 4) DETECTORS 
\newcommand{\ITS}          {\rm{ITS}\xspace}
\newcommand{\TOF}          {\rm{TOF}\xspace}
\newcommand{\ZDC}          {\rm{ZDC}\xspace}
\newcommand{\ZDCs}         {\rm{ZDCs}\xspace}
\newcommand{\ZNA}          {\rm{ZNA}\xspace}
\newcommand{\ZNC}          {\rm{ZNC}\xspace}
\newcommand{\SPD}          {\rm{SPD}\xspace}
\newcommand{\SDD}          {\rm{SDD}\xspace}
\newcommand{\SSD}          {\rm{SSD}\xspace}
\newcommand{\TPC}          {\rm{TPC}\xspace}
\newcommand{\TRD}          {\rm{TRD}\xspace}
\newcommand{\VZERO}        {\rm{V0}\xspace}
\newcommand{\VZEROA}       {\rm{V0A}\xspace}
\newcommand{\VZEROC}       {\rm{V0C}\xspace}
\newcommand{\Vdecay} 	   {\ensuremath{V^{0}}\xspace}

% 4) PARTICLE SPECIES 
\newcommand{\hadrons}      {\ensuremath{\mathrm{h}^{\pm}}\xspace}
\newcommand{\pion}         {\ensuremath{\pi}\xspace}
\newcommand{\kaon}         {\ensuremath{\textrm{K}}\xspace}
\newcommand{\pr}           {\ensuremath{\textrm{p}}\xspace}
\newcommand{\prx}          {\ensuremath{\mathrm{p}(\overline{\mathrm{p}}})\xspace}
\newcommand{\ee}           {\ensuremath{e^{+}e^{-}}} 
\newcommand{\pip}          {\ensuremath{\pi^{+}}\xspace}
\newcommand{\pim}          {\ensuremath{\pi^{-}}\xspace}
\newcommand{\kapm}         {\ensuremath{\mathrm{K}^{\pm}}}
\newcommand{\kap}          {\ensuremath{\rm{K}^{+}}\xspace}
\newcommand{\kam}          {\ensuremath{\rm{K}^{-}}\xspace}
\newcommand{\pbar}         {\ensuremath{\rm\overline{p}}\xspace}
\newcommand{\kzero}        {\ensuremath{{\rm K}^{0}_{\rm{S}}}\xspace}
\newcommand{\lmb}          {\ensuremath{\Lambda}\xspace}
\newcommand{\almb}         {\ensuremath{\overline{\Lambda}}\xspace}
\newcommand{\Om}           {\ensuremath{\Omega^-}\xspace}
\newcommand{\Mo}           {\ensuremath{\overline{\Omega}^+}\xspace}
\newcommand{\X}            {\ensuremath{\Xi^-}\xspace}
\newcommand{\Ix}           {\ensuremath{\overline{\Xi}^+}\xspace}
\newcommand{\Xis}          {\ensuremath{\Xi^{\pm}}\xspace}
\newcommand{\Oms}          {\ensuremath{\Omega^{\pm}}\xspace}
\newcommand{\degree}       {\ensuremath{^{\rm o}}\xspace}

% Particle ratios
\newcommand{\ktopi}        {\ensuremath{\mathrm{K}/\pi}\xspace}
\newcommand{\ptopi}        {\ensuremath{\mathrm{p}/\pi}\xspace}

% PID 
\newcommand{\nsigma}       {\ensuremath{\mathrm{n}_{\sigma}}\xspace}

